One-shot Active Learning Based on Lewis Weight Sampling for Multiple Deep Models

Active learning (AL) for multiple target models aims to reduce labeled data querying while effectively training multiple models concurrently. Existing AL algorithms often rely on iterative model training, which can be computationally expensive, particularly for deep models. In this paper, we propose a one-shot AL method to address this challenge, which performs all label queries without repeated model training. Specifically, we extract different representations of the same dataset using distinct network backbones, and actively learn the linear prediction layer on each representation via an $\ell_p$-regression formulation. The regression problems are solved approximately by sampling and reweighting the unlabeled instances based on their maximum Lewis weights across the representations. An upper bound on the number of samples needed is provided with a rigorous analysis for $p\in [1, +\infty)$. Experimental results on 11 benchmarks show that our one-shot approach achieves competitive performances with the state-of-the-art AL methods for multiple target models.

==> emp_obs.tex <==
\section{An Empirical Observation}\label{sec:empobs}

To address the challenges of distinct representations from multiple deep models, one solution is to sample the unlabeled instances by their maximum Lewis weight among different representations.
Recall that the sample size is proportional to the sum of the sampling probabilities, this strategy will not save the number of queries if the sum of the maximum Lewis weights is $k$ times larger than that of a single regression problem.
Therefore, we would like first to examine the sum of maximum Lewis weights across representations as it will determine the potential query savings.
In the following empirical studies, we mainly consider the case of $p=2$ (i.e., squared loss), which is a common choice in training deep regression models. 

\begin{figure*}[!ht]
	\centering
	\subfloat[MNIST]{
		\includegraphics[width=\threefigsmargin]{figures/mnist.pdf}
	}
	\subfloat[Kuzushiji-MNIST]{
		\includegraphics[width=\threefigsmargin]{figures/kmnist.pdf}
	}
	\subfloat[Fashion-MNIST]{
		\includegraphics[width=\threefigsmargin]{figures/fmnist.pdf}
	}
	\subfloat[EMNIST-digits]{
		\includegraphics[width=\threefigsmargin]{figures/emnistdig.pdf}
	}
	\subfloat[EMNIST-letters]{
		\includegraphics[width=\threefigsmargin]{figures/emnistlet.pdf}
	}
	\subfloat[SVHN]{
		\includegraphics[width=\threefigsmargin]{figures/svhn.pdf}
	}\\[-2.5ex]
	\subfloat[CIFAR-10]{
		\includegraphics[width=\threefigsmargin]{figures/cifar10.pdf}
	}
	\subfloat[Biwi]{
		\includegraphics[width=\threefigsmargin]{figures/biwi.pdf}
	}
	\subfloat[FLD]{
		\includegraphics[width=\threefigsmargin]{figures/flw.pdf}
	}
	\caption{The trends of the sum of the maximum Lewis weights with $p=2$ among multiple representations as the number of deep models increases.}\label{fig:observation}
\end{figure*}

\textbf{Empirical Settings. } We employ 50 distinct network architectures to generate the representations of the dataset. These architectures are published by a recent NAS method OFA \citep{cai2019once} for accommodating diverse resource-constraint devices, ranging from NVIDIA Tesla V100 GPU to mobile devices. It aligns well with our problem setting.
We conduct experiments on 9 datasets, including 7 classification benchmarks:  MNIST \citep{lecun1998gradient}, Fashion-MNIST \citep{xiao2017/online}, Kuzushiji-MNIST \citep{clanuwat2018deep}, SVHN \citep{netzer2011reading}, EMNIST-digits and EMNIST-letters \citep{CohenATS17}, CIFAR-10 \citep{krizhevsky2009learning}; and 2 regression benchmarks: Biwi \citep{fanelli2013random} and FLD \citep{sun2013deep}.  The specifications of the datasets and the details of model configurations are deferred to the Section~\ref{sec:detailsetting}.
For each dataset, we randomly sample 3000 instances to train the models with 20 epochs, then extract features for the whole dataset and calculate their Lewis weights. We use the squared loss in model training and keep all other settings the same as the OFA project. Figure~\ref{fig:observation} shows the theoretical upper bound and the exact values of the sum of the maximum Lewis weight of each instance across different representations.

\textbf{Results. } We first plot the upper bound of the sum of the maximum Lewis weights across multiple representations as the number of models increases. 
For matrices $A^1,\dots,A^k$ of $n$ rows, it clearly holds that $\sum_i \max_j w_i(A^j) \leq \min\{\sum_i\sum_j  w_i(A^j), \sum_i 1\} \leq \min\{\sum_i \rk(A^j), n\}$. This upper bound is plotted in red color, which grows almost linearly until it reaches the number of instances $n$.

\begin{wrapfigure}[24]{l}{0.55\textwidth}
	\begin{minipage}{0.55\textwidth}
		\vspace{-25pt}
		\begin{algorithm}[H]
			\caption{The Proposed Algorithm. }
			\label{alg:max_lewis_weight}
			\begin{algorithmic}[1]
				\Require{Feature matrices of labeled and unlabeled instances $L^j, U^j$ ($j=1,\dots,k$), query budget $\tau $.}
				\Ensure{Trained linear models $\tilde{\bm{\theta}}^1, \dots, \tilde{\bm{\theta}}^k$.}
				\INPUT {$\bm{p}, \bar{\bm{y}} \gets \text{zero vector of length } n_u$; $\cQ \gets$ an empty list; $m \gets 0$}
				% \State{$\cQ \gets$ an empty list}
				% \State{$m \gets 0$}
				\State{${p}_i \gets \max_{1 \leq j \leq k}{w_i(U^j)}$ for $i=1,\dots,n_u$}
				\State{${p}_i \gets {p}_i/\norm{\bm{p}}_1$ for $i=1,\dots,n_u$}
				% \State{$\bm{w} \gets$ overestimate $\bm{w}$ so that $\sum_{i=1}^{n_u}\bm{w}_i=\tau$} 
				\While{ $\cQ$ has fewer than $\tau$ distince elements}\label{line:sample-start}
				\State{$q \gets$ sample a number from $[n_u]$ with replace-\newline
                    \hspace*{3.27em} ment with probability ${p}_1, \dots, {p}_{n_u}$}
				\State{$m \gets m+1$}
				\State{append $q$ to $\cQ$}
				\If{the label of $q$-th unlabeled instance is \newline \hspace*{2.1em} unknown}
				\State{$\bar{{y}}_q \gets$ query the label of $q$-th unlabeled \newline
                        \hspace*{5.27em} instance}
				\EndIf
				\EndWhile\label{line:sample-end}
				\State{$S \gets $ zero matrix with shape $(n_l+m) \times (n_l+n_u)$}
				\State $S_{i,i} \gets 1$ for $i=1, \dots, n_l$
				\State{$S_{i+n_l,\cQ_i+n_l} \gets \sqrt{1/(m\cdot p_{\cQ_i})}$ for $i=1,\dots, m$}
				
				\State{$\bm{y} \gets [y_1, \dots, y_{n_l}, \bar{\bm{y}}]^T$}
				
				\For{$j=1,...,k$}
				\State{$A^j \gets \big[\begin{smallmatrix} L^j \\ U^j \end{smallmatrix}\big]$}
				\State{$\tilde{\bm{\theta}}^j \gets \arg\min_{x\in E}\norm{Sf(A^j\bm{\theta})-S\bm{y}}_p^p$, where \newline
                \hspace*{3.87em} $E = \{\bm{\theta}:\norm{SA^j \bm{\theta}}_p^p\leq \frac{1}{\eps L^p }\norm{S\bm{y}}_p^p\}$ }
				\EndFor
				\State{\Return $\tilde{\bm{\theta}}^1, \dots, \tilde{\bm{\theta}}^k$}
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
\end{wrapfigure}

\vspace{-50pt}

We examine the exact values of the sum of maximum Lewis weights across multiple representations. All figures show that the exact sum grows very slowly as the number of models increases. This suggests highly consistent discrimination power of most instances across different representations, as the Lewis weight when $p=2$ is exactly the leverage score, which measures how hard an instance can be linearly represented by others. Therefore, a small number of discriminating examples suffices to effectively train multiple models. Lewis weights also provide a possible direction to interpret the behavior of deep representation learning, as prior works have not discovered any simple form of correlation among the diverse representations obtained by different model architectures
\citep{kornblith2019similarity,nguyen2020wide}.

